A stable splitting of factorisation homology of generalised surfaces

For a manifold $W$ and an $E_d$-algebra $A$, the factorisation homology $\int_W A$ can be seen as a generalisation of the classical configuration space of labelled particles in $W$. It carries an action by the diffeomorphism group $\mathrm{Diff}_\partial(W)$, and for the generalised surfaces $W_{g,1}:=(\#^g S^n\times S^n)\setminus\mathring D{}^{2n}$, we have stabilisation maps among the quotients $\int_{W_{g,1}} A\,/\!/\,\mathrm{Diff}_\partial(W_{g,1})$ which increase the genus $g$. In the case where a highly-connected tangential structure $\theta$ is taken into account, we describe its stable homology in terms of the iterated bar construction $\mathrm{B}^{2n}A$ and a tangential Thom spectrum $\mathrm{MT}\theta$. We also consider the question of homological stability.

==> preamble-bib.tex <==
%

\usepackage[backend      = biber,
            style        = alphabetic,
            maxbibnames  = 9,
            maxcitenames = 9,
            doi          = false,
            bibencoding  = utf8,
            datamodel    = ext-eprint]{biblatex}

%
\DefineBibliographyExtras{british}{%
  \renewcommand{\finalandcomma}{,}
}

%
\makeatletter
\DeclareFieldFormat{eprint:arxiv}{%
  arXiv\addcolon\space
  \ifhyperref
    {\href{http://arxiv.org/\abx@arxivpath/#1}{%
       \nolinkurl{#1}%
       \iffieldundef{eprintclass}
     {}
     {\addspace\textsf{\mkbibbrackets{\thefield{eprintclass}}}}}}
    {\nolinkurl{#1}
     \iffieldundef{eprintclass}
       {}
       {\addspace\textsf{\mkbibbrackets{\thefield{eprintclass}}}}}}%
\makeatother

%
%
\DefineBibliographyExtras{british}{\protected\def\bibrangedash{\nobreakdash--}}
\DefineBibliographyExtras{ngerman}{\protected\def\bibrangedash{\nobreakdash--}}

\AtBeginBibliography{\footnotesize}

\bibliography{bibliography.bib}


==> preamble-custom.tex <==
\usepackage[size=tiny]{todonotes}

%
\newcommand{\dE} [2][]{\smash{E_{\smash{#2}}   \ifx\\#1\\\else^{#1}\fi}}
\newcommand{\dF} [2][]{\smash{F_{\smash{#2}}   \ifx\\#1\\\else^{#1}\fi}}
\newcommand{\dbE}[2][]{\smash{\bbE_{\smash{#2}}\ifx\\#1\\\else^{#1}\fi}}
\newcommand{\dbF}[2][]{\smash{\bbF_{\smash{#2}}\ifx\\#1\\\else^{#1}\fi}}
\newcommand{\udbE}[2][]{\smash{\ul{\bbE}_{\smash{#2}}\ifx\\#1\\\else^{#1}\fi}}
\newcommand{\dW} [2][]{\smash{W_{\smash{#2}}   \ifx\\#1\\\else^{#1}\fi}}
\newcommand{\dbW}[2][]{\smash{\bbW_{\smash{#2}}\ifx\\#1\\\else^{#1}\fi}}
\newcommand{\dsW}[2][]{\smash{\caW_{\smash{#2}}\ifx\\#1\\\else^{#1}\fi}}
\newcommand{\mdE}[2][]{\smash{\bbD_{\smash{#2}}\ifx\\#1\\\else^{#1}\fi}}

%
\newcommand{\h}[1]{{\smash{\on{h}#1}}}

%
\newcommand{\SO}   {\on{SO}}
\newcommand{\B}    {\on{B}}
\newcommand{\E}    {\on{E}}
\newcommand{\MT}   {\on{MT}}
\newcommand{\Emb}  {\on{Emb}}
\newcommand{\Bun}  {\on{Bun}}
\renewcommand{\Top}{\on{Top}}
\newcommand{\Comp} {\on{Comp}{}}
\renewcommand{\Alg}{\on{Alg}{}}
\newcommand{\Sp}   {\on{Sp}{}}
\newcommand{\Fun}  {\on{Fun}}
\newcommand{\ulB}  {\ul{\B}}
\newcommand{\ulE}  {\ul{\E}}
\newcommand{\tbE}  {\tilde\bbE}
\newcommand{\conn} {{\mathrm{cn}}}
\newcommand{\Map}  {\on{Map}{}}
\newcommand{\Fin}  {\on{Fin}{}}
\newcommand{\Cat}  {\on{Cat}}
\newcommand{\Op}   {\on{Op}{}}
\newcommand{\cN}   {\on{N}}
\newcommand{\colim}{\on{colim}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\Fr}   {\on{Fr}}
\newcommand{\BO}{\mathrm{BO}}
\newcommand{\elll}{\ell}

\usepackage{marginnote}
%
%

\usetikzlibrary{patterns}


==> preamble-env.tex <==
%

%
%
%
\makeatletter
  \@ifpackageloaded{amsthm}{}{\usepackage{amsthm}}
\makeatother

%
%
%
\usepackage[capitalise,noabbrev]{cleveref}

\theoremstyle{plain}
\newtheorem{theo}   {Theorem}[section]
\newtheorem{thm}    [theo]{Theorem}
\newtheorem{lem}    [theo]{Lemma}
\newtheorem{prop}   [theo]{Proposition}
\newtheorem{cor}    [theo]{Corollary}
\newtheorem{conj}   [theo]{Conjecture}

\theoremstyle{definition}
\newtheorem{defi}   [theo]{Definition}
\newtheorem{probl}  [theo]{Problem}
\newtheorem{expl}   [theo]{Example}
\newtheorem{nota}   [theo]{Notation}
\newtheorem{constr} [theo]{Construction}
\newtheorem{outl}   [theo]{Outlook}
\newtheorem{exer}   [theo]{Exercise}
\newtheorem{rem}    [theo]{Remark} %
\newtheorem{rmk}    [theo]{Remark}
\newtheorem{rmd}    [theo]{Reminder}
\newtheorem{idea}   [theo]{Idea}

\crefname{prop}{Proposition}{Propositions}
\crefname{theo}{Theorem}  {Theorems}
\crefname{cor} {Corollary}{Corollaries}

%
%
%
%
%

%
\newlength{\intendedDistance}

%
\newcommand{\wrap}[1]{
  \setlength{\intendedDistance}{\lastskip}\addvspace{-\lastskip}
  #1
  \addvspace{\intendedDistance}
}

%
\newenvironment{t-figure}{
  \setlength{\intendedDistance}{\lastskip}\addvspace{-\lastskip}
  \begin{figure}[t]
  }{
  \end{figure}
  \addvspace{\intendedDistance}
}

%
\newenvironment{t-table}{
  \setlength{\intendedDistance}{\lastskip}\addvspace{-\lastskip}  
  \begin{table}[t]
  \centering
  }{
  \end{table}
  \addvspace{\intendedDistance}
}


==> preamble-math.tex <==
%

%
\usepackage{amssymb,amsmath} %
\usepackage{mathtools}       %
\usepackage{stmaryrd}        %

%
\usepackage{tikz-cd}
\usepackage{tikz}
\usetikzlibrary{arrows,calc}

%
\usepackage{scalerel}

%
\let \le       \leqslant
\let \ge       \geqslant
\let \leq      \leqslant
\let \geq      \geqslant
\let \setminus \smallsetminus
\let \emptyset \varnothing
\let \epsilon  \varepsilon
%

%
\newcommand{\bm} [1]{\mathbold{#1}}

%
\newcommand{\ol} [1]{\overline{#1}}
\newcommand{\on} [1]{\mathrm{#1}}

%
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}
\renewcommand{\bigl}{\mathopen\big}
\renewcommand{\bigr}{\mathclose\big}

%
\newcommand{\lla}[1]{\mathopen{}\left\langle #1 \right\rangle\mathclose{}}      %
\newcommand{\ula}[1]{\langle #1\rangle}                                         %
\newcommand{\llb}[1]{\mathopen{}\left\llbracket #1\right\rrbracket\mathclose{}} %
\newcommand{\ulb}[1]{\mathopen{}\left\llbracket #1\right\rrbracket\mathclose{}} %

%
\newcommand{\GL} {\on{GL}}
\newcommand{\pr} {\on{pr}}
\newcommand{\ob} {\on{ob}}
\newcommand{\sg} {\on{sg}}
\newcommand{\im} {\on{im}}
\newcommand{\op} {{\on{op}}} %
\newcommand{\Aut}{\on{Aut}}
\newcommand{\Hom}{\on{Hom}}
\newcommand{\map}{\on{map}}
\newcommand{\Id} {\on{id}}   %

%
\newcommand*\lon{%
        \nobreak
        \mskip6mu plus1mu
        \mathpunct{}%
        \nonscript
        \mkern-\thinmuskip
        {:}%
        \mskip2mu
        \relax
}

%
\newcommand{\Top}{\mathbf{Top}}
\newcommand{\Sig}{\mathbf{\Sigma}}
\newcommand{\Del}{\mathbf{\Delta}}
\newcommand{\Set}{\mathbf{Set}}
\newcommand{\Mod}{\mathbf{Mod}}
\newcommand{\Alg}{\mathbf{Alg}}

%
\newcommand{\bEn}{\mathbb{1}}
\newcommand{\RP}{\R\mathrm{P}}
\newcommand{\CP}{\C\mathrm{P}}
\newcommand{\Diff}{\on{Diff}{}}
\newcommand{\hAut}{\on{hAut}}
\newcommand{\dcup}{\,\dot\cup\,}
\newcommand{\swr}{\kern.6px\wr\kern.6px}

%
\DeclareSymbolFont{eulargesymbols}{U}{zeuex}{m}{n}
\DeclareMathSymbol{\intop}{\mathop}{eulargesymbols}{"52}

%
\def\centerarc[#1](#2)(#3:#4:#5)%
    { \draw[#1] ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5); }

%

%
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

%
\usepackage{letltxmacro}
\LetLtxMacro\orgvdots\vdots
\LetLtxMacro\orgddots\ddots
\makeatletter
\DeclareRobustCommand\vdots{%
  \mathpalette\@vdots{}%
}
\newcommand*{\@vdots}[2]{%
  %
  %
  \sbox0{$#1\cdotp\cdotp\cdotp\m@th$}%
  \sbox2{$#1.\m@th$}%
  \vbox{%
    \dimen@=\wd0 %
    \advance\dimen@ -3\ht2 %
    \kern.5\dimen@
    %
    \dimen@=\wd2 %
    \advance\dimen@ -\ht2 %
    \dimen2=\wd0 %
    \advance\dimen2 -\dimen@
    \vbox to \dimen2{%
      \offinterlineskip
      \copy2 \vfill\copy2 \vfill\copy2 %
    }%
  }%
}
\makeatother

%
\DeclareFontFamily{OMS}{zplm}{
   \skewchar\font=48 %
   \fontdimen 9\font=0.34\fontdimen6\font
   \fontdimen 8\font=0.84\fontdimen6\font
}
\DeclareFontShape{OMS}{zplm}{m}{n}{<-> zplmr7y}{}
\DeclareFontShape{OMS}{zplm}{b}{n}{<-> zplmb7y}{}
\DeclareFontShape{OMS}{zplm}{bx}{n}{<->ssub * zplm/b/n}{}

%
%

%
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%
\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

%
\newcommand{\caA}{\mathcal{A}}
\newcommand{\caB}{\mathcal{B}}
\newcommand{\caC}{\mathcal{C}}
\newcommand{\caD}{\mathcal{D}}
\newcommand{\caE}{\mathcal{E}}
\newcommand{\caF}{\mathcal{F}}
\newcommand{\caG}{\mathcal{G}}
\newcommand{\caH}{\mathcal{H}}
\newcommand{\caI}{\mathcal{I}}
\newcommand{\caJ}{\mathcal{J}}
\newcommand{\caK}{\mathcal{K}}
\newcommand{\caL}{\mathcal{L}}
\newcommand{\caM}{\mathcal{M}}
\newcommand{\caN}{\mathcal{N}}
\newcommand{\caO}{\mathcal{O}}
\newcommand{\caP}{\mathcal{P}}
\newcommand{\caQ}{\mathcal{Q}}
\newcommand{\caR}{\mathcal{R}}
\newcommand{\caS}{\mathcal{S}}
\newcommand{\caT}{\mathcal{T}}
\newcommand{\caU}{\mathcal{U}}
\newcommand{\caV}{\mathcal{V}}
\newcommand{\caW}{\mathcal{W}}
\newcommand{\caX}{\mathcal{X}}
\newcommand{\caY}{\mathcal{Y}}
\newcommand{\caZ}{\mathcal{Z}}

%
\newcommand{\scA}{\mathscr{A}}
\newcommand{\scB}{\mathscr{B}}
\newcommand{\scC}{\mathscr{C}}
\newcommand{\scD}{\mathscr{D}}
\newcommand{\scE}{\mathscr{E}}
\newcommand{\scF}{\mathscr{F}}
\newcommand{\scG}{\mathscr{G}}
\newcommand{\scH}{\mathscr{H}}
\newcommand{\scI}{\mathscr{I}}
\newcommand{\scJ}{\mathscr{J}}
\newcommand{\scK}{\mathscr{K}}
\newcommand{\scL}{\mathscr{L}}
\newcommand{\scM}{\mathscr{M}}
\newcommand{\scN}{\mathscr{N}}
\newcommand{\scO}{\mathscr{O}}
\newcommand{\scP}{\mathscr{P}}
\newcommand{\scQ}{\mathscr{Q}}
\newcommand{\scR}{\mathscr{R}}
\newcommand{\scS}{\mathscr{S}}
\newcommand{\scT}{\mathscr{T}}
\newcommand{\scU}{\mathscr{U}}
\newcommand{\scV}{\mathscr{V}}
\newcommand{\scW}{\mathscr{W}}
\newcommand{\scX}{\mathscr{X}}
\newcommand{\scY}{\mathscr{Y}}
\newcommand{\scZ}{\mathscr{Z}}

%
\newcommand{\sca}{\mathscr{a}}
\newcommand{\scb}{\mathscr{b}}
\newcommand{\scc}{\mathscr{c}}
\newcommand{\scd}{\mathscr{d}}
\newcommand{\sce}{\mathscr{e}}
\newcommand{\scf}{\mathscr{f}}
\newcommand{\scg}{\mathscr{g}}
\newcommand{\sch}{\mathscr{h}}
\newcommand{\sci}{\mathscr{i}}
\newcommand{\scj}{\mathscr{j}}
\newcommand{\sck}{\mathscr{k}}
\newcommand{\scl}{\mathscr{l}}
\newcommand{\scm}{\mathscr{m}}
\newcommand{\scn}{\mathscr{n}}
\newcommand{\sco}{\mathscr{o}}
\newcommand{\scp}{\mathscr{p}}
\newcommand{\scq}{\mathscr{q}}
\newcommand{\scr}{\mathscr{r}}
\newcommand{\scs}{\mathscr{s}}
\newcommand{\sct}{\mathscr{t}}
\newcommand{\scu}{\mathscr{u}}
\newcommand{\scv}{\mathscr{v}}
\newcommand{\scw}{\mathscr{w}}
\newcommand{\scx}{\mathscr{x}}
\newcommand{\scy}{\mathscr{y}}
\newcommand{\scz}{\mathscr{z}}

%
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

%
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

%
\newcommand{\bmA}{\bm{A}}
\newcommand{\bmB}{\bm{B}}
\newcommand{\bmC}{\bm{C}}
\newcommand{\bmD}{\bm{D}}
\newcommand{\bmE}{\bm{E}}
\newcommand{\bmF}{\bm{F}}
\newcommand{\bmG}{\bm{G}}
\newcommand{\bmH}{\bm{H}}
\newcommand{\bmI}{\bm{I}}
\newcommand{\bmJ}{\bm{J}}
\newcommand{\bmK}{\bm{K}}
\newcommand{\bmL}{\bm{L}}
\newcommand{\bmM}{\bm{M}}
\newcommand{\bmN}{\bm{N}}
\newcommand{\bmO}{\bm{O}}
\newcommand{\bmP}{\bm{P}}
\newcommand{\bmQ}{\bm{Q}}
\newcommand{\bmR}{\bm{R}}
\newcommand{\bmS}{\bm{S}}
\newcommand{\bmT}{\bm{T}}
\newcommand{\bmU}{\bm{U}}
\newcommand{\bmV}{\bm{V}}
\newcommand{\bmW}{\bm{W}}
\newcommand{\bmX}{\bm{X}}
\newcommand{\bmY}{\bm{Y}}
\newcommand{\bmZ}{\bm{Z}}

%
\newcommand{\frA}{\mathfrak{A}}
\newcommand{\frB}{\mathfrak{B}}
\newcommand{\frC}{\mathfrak{C}}
\newcommand{\frD}{\mathfrak{D}}
\newcommand{\frE}{\mathfrak{E}}
\newcommand{\frF}{\mathfrak{F}}
\newcommand{\frG}{\mathfrak{G}}
\newcommand{\frH}{\mathfrak{H}}
\newcommand{\frI}{\mathfrak{I}}
\newcommand{\frJ}{\mathfrak{J}}
\newcommand{\frK}{\mathfrak{K}}
\newcommand{\frL}{\mathfrak{L}}
\newcommand{\frM}{\mathfrak{M}}
\newcommand{\frN}{\mathfrak{N}}
\newcommand{\frO}{\mathfrak{O}}
\newcommand{\frP}{\mathfrak{P}}
\newcommand{\frQ}{\mathfrak{Q}}
\newcommand{\frR}{\mathfrak{R}}
\newcommand{\frS}{\mathfrak{S}}
\newcommand{\frT}{\mathfrak{T}}
\newcommand{\frU}{\mathfrak{U}}
\newcommand{\frV}{\mathfrak{V}}
\newcommand{\frW}{\mathfrak{W}}
\newcommand{\frX}{\mathfrak{X}}
\newcommand{\frY}{\mathfrak{Y}}
\newcommand{\frZ}{\mathfrak{Z}}

%
\newcommand{\fra}{\mathfrak{a}}
\newcommand{\frb}{\mathfrak{b}}
\newcommand{\frc}{\mathfrak{c}}
\newcommand{\frd}{\mathfrak{d}}
\newcommand{\fre}{\mathfrak{e}}
\newcommand{\frf}{\mathfrak{f}}
\newcommand{\frg}{\mathfrak{g}}
\newcommand{\frh}{\mathfrak{h}}
\newcommand{\fri}{\mathfrak{i}}
\newcommand{\frj}{\mathfrak{j}}
\newcommand{\frk}{\mathfrak{k}}
\newcommand{\frl}{\mathfrak{l}}
\newcommand{\frm}{\mathfrak{m}}
\newcommand{\frn}{\mathfrak{n}}
\newcommand{\fro}{\mathfrak{o}}
\newcommand{\frp}{\mathfrak{p}}
\ifdefined\frq\renewcommand{\frq}{\mathfrak{q}}\else \newcommand{\frq}{\mathfrak{q}}\fi
\newcommand{\frr}{\mathfrak{r}}
\newcommand{\frs}{\mathfrak{s}}
\newcommand{\frt}{\mathfrak{t}}
\newcommand{\fru}{\mathfrak{u}}
\newcommand{\frv}{\mathfrak{v}}
\newcommand{\frw}{\mathfrak{w}}
\newcommand{\frx}{\mathfrak{x}}
\newcommand{\fry}{\mathfrak{y}}
\newcommand{\frz}{\mathfrak{z}}

%
\newcommand{\tA}{\tilde{A}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tC}{\tilde{C}}
\newcommand{\tD}{\tilde{D}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tI}{\tilde{I}}
\newcommand{\tJ}{\tilde{J}}
\newcommand{\tK}{\tilde{K}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tM}{\tilde{M}}
\newcommand{\tN}{\tilde{N}}
\newcommand{\tO}{\tilde{O}}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tQ}{\tilde{Q}}
\newcommand{\tR}{\tilde{R}}
\newcommand{\tS}{\tilde{S}}
\newcommand{\tT}{\tilde{T}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tX}{\tilde{X}}
\newcommand{\tY}{\tilde{Y}}
\newcommand{\tZ}{\tilde{Z}}


%
%
%
%
%
%
%
%

\usepackage{nicefrac}


==> preamble.tex <==
%
\makeatletter
\@ifclassloaded{scrlttr2}{%
  \KOMAoptions{fontsize=11pt,parskip,fromalign=right,foldmarks=TBMpL,enlargefirstpage}
  \setkomavar{backaddressseparator}{~\textbullet~}
  \renewcommand*{\raggedsignature}{\raggedright}
}{\KOMAoptions{headings=standardclasses,numbers=enddot}}
\makeatother

%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

%
\usepackage{babel}
\usepackage{csquotes} %

%
\usepackage[cleanlook]{isodate}

%
\usepackage{lmodern}

%
%
\usepackage[osf,sc]{mathpazo}

%
\newcommand{\LF}[1]{{\fontfamily{pplx}\selectfont #1}}

%
\usepackage{myT1classico}

%
\usepackage[scaled=.85]{beramono}

%
\usepackage{setspace}
\setstretch{1.07}
\renewcommand{\arraystretch}{1.07} %

%
\usepackage{ellipsis} %
\usepackage[babel,tracking=true]{microtype}

%
\makeatletter
\@ifclassloaded{scrlttr2}{%
   \addtokomafont{refvalue}   {\fontfamily{pplx}\selectfont}
   \addtokomafont{fromaddress}{\fontfamily{pplx}\selectfont}
   \addtokomafont{addressee}  {\fontfamily{pplx}\selectfont}
   \addtokomafont{toaddress}  {\fontfamily{pplx}\selectfont}
}
\makeatother

%
\makeatletter
\@ifpackagelater{microtype}{2020/12/08}
  {\microtypesetup{nopatch=footnote}}
  {}
\makeatother

%
\UseMicrotypeSet[tracking]{smallcaps}
\SetTracking{encoding=*,shape=sc}{30}

%
\makeatletter
  \widowpenalty=\@M
\makeatother

%
\relpenalty=10000
\binoppenalty=10000

%
\everypar=\expandafter{\the\everypar\looseness=-1}

%
\raggedbottom

%
\usepackage{relsize}
\newcommand{\acr}[1]{\texorpdfstring{\textls[40]{\textsc{\MakeLowercase{#1}}}}{#1}}

%
\usepackage[shortlabels]{enumitem}

%
%
%
\let\COld\C

%
\usepackage{graphicx}
\usepackage[margin    =20pt,
            font      ={footnotesize,stretch=1.06},
            format    =plain,
            labelsep  =period,
            labelfont =bf]{caption}
  
%
\let\C\COld

%
\usepackage{booktabs}
  
%
\usepackage{xcolor}

%
%
\IfFileExists{preamble-math.tex}  {\input{preamble-math.tex}}  {}
\IfFileExists{preamble-bib.tex}   {\input{preamble-bib.tex}}   {}
\IfFileExists{preamble-music.tex} {\input{preamble-music.tex}} {}
\IfFileExists{preamble-custom.tex}{\input{preamble-custom.tex}}{}

%
\usepackage{footmisc}
\renewcommand{\footnotelayout}{\setstretch{1.06}}
\setlength{\footnotemargin}{1em}

%
\addtokomafont{pagehead}{\fontfamily{ppl}\selectfont}

%
\setkomafont{descriptionlabel}{\scshape}

%
%
%
\newcommand{\pazofrac}[2]%
  {\leavevmode\kern.1em\raise.65ex\hbox{\scriptsize #1}%
   \kern-.125em/\kern-.125em\lower-.05ex\hbox{\scriptsize #2}}

%
\usepackage{etoolbox}
\ifundef{\abstract}{}{
  \patchcmd{\abstract}{\quotation}{\quotation\noindent\ignorespaces}{}{}}

%
%
\usepackage[pdfusetitle,%
            bookmarksnumbered=true,%
            unicode,%
            hidelinks]{hyperref}
            
%
%
\let\mailfont\textsf
\urlstyle{sf} 

%
\newcommand{\mail}[1]{\upshape\href{mailto:#1}{\mailfont{#1}}}

%
\hypersetup{
  colorlinks,
  linkcolor={black!45!red},   %
  citecolor={black!55!green}, %
  urlcolor ={black!45!blue}   %
}

%
\IfFileExists{preamble-env.tex}{\input{preamble-env.tex}}{}

%
\newcommand{\addr}[2]{%
  \paragraph{#1}
  \LF{#2}
} 

%
\newcommand{\makesmalltoc}{
  \RedeclareSectionCommand[tocbeforeskip=3pt]{section}
  \setkomafont{sectionentry}{\normalfont}
  \setcounter{tocdepth}{1}
  \tableofcontents
}

%
%
%
\makeatletter
\newcommand{\makesmalltitle}[1][]{
  \thispagestyle{empty}
  \begin{center}
    \ifthenelse{\equal{\@subject}{}}{}{\textbf{\@subject}\\}%
    \Large\textbf{\@title}\\
    \large%
    \ifthenelse{\equal{#1}{}}{%
       \ifthenelse{\equal{\@subtitle}{}}{%
          \@author%
       }{\@subtitle}%
    }{#1}\vspace*{\baselineskip}
  \end{center}
}
\makeatother 

%
\KOMAoptions{DIV=10}

